DGSAC: Density Guided Sampling and Consensus

Robust multiple model fitting plays a crucial role in many computer vision applications. Unlike single model fitting problems, the multi-model fitting has additional challenges. The unknown number of models and the inlier noise scale are the two most important of them, which are in general provided by the user using ground-truth or some other auxiliary information. Mode seeking/ clustering-based approaches crucially depend on the quality of model hypotheses generated. While preference analysis based guided sampling approaches have shown remarkable performance, they operate in a time budget framework, and the user provides the time as a reasonable guess. In this paper, we deviate from the mode seeking and time budget framework. We propose a concept called Kernel Residual Density (KRD) and apply it to various components of a multiple-model fitting pipeline. The Kernel Residual Density act as a key differentiator between inliers and outliers. We use KRD to guide and automatically stop the sampling process. The sampling process stops after generating a set of hypotheses that can explain all the data points. An explanation score is maintained for each data point, which is updated on-the-fly. We propose two model selection algorithms, an optimal quadratic program based, and a greedy. Unlike mode seeking approaches, our model selection algorithms seek to find one representative hypothesis for each genuine structure present in the data. We evaluate our method (dubbed as DGSAC) on a wide variety of tasks like planar segmentation, motion segmentation, vanishing point estimation, plane fitting to 3D point cloud, line, and circle fitting, which shows the effectiveness of our method and its unified nature.

==> hom_hyp_gen.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% %\scriptsize
% \setlength{\tabcolsep}{2pt}
% %\fontsize{9}{11}\selectfont
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%                                                               &     &      &      &      &      \\ \hline
%                                                               &     &      &      &      &      \\ \hline
% \multirow{4}{*}{
% \begin{tabular}{c{5cm}}
%      \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
%      Barrsmith, N=600
%      \vspace{-0.24cm}\\
%      O=65.4, \tau=3, $S=[50,20,23,34,45]$\\
% \end{tabular}
% } & abc & 620  & 218  & 55   & 34   \\ \cline{2-6} 
%                                                               & def & 0.10 & 0.17 & 0.16 & 0.87 \\ \cline{2-6} 
%                                                               & ghi & 0.06 & 0.08 & 0.08 & 0.85 \\ \cline{2-6} 
%                                                               & jkl & 1    & 2    & 2    & 2    \\ \hline
% \multirow{4}{*}{}                                              &     & 463  & 201  & 61   & 57   \\ \cline{2-6} 
%                                                               &     & 0.18 & 0.27 & 0.45 & 0.96 \\ \cline{2-6} 
%                                                               &     & 0.17 & 0.21 & 0.31 & 1.00 \\ \cline{2-6} 
%                                                               &     & 2    & 2    & 2    & 2    \\ \hline
% \multirow{4}{*}{}                                              &     & 611  & 231  & 56   & 64   \\ \cline{2-6} 
%                                                               &     & 0.16 & 0.24 & 0.28 & 0.82 \\ \cline{2-6} 
%                                                               &     & 0.12 & 0.12 & 0.15 & 0.82 \\ \cline{2-6} 
%                                                               &     & 2    & 3    & 2    & 3    \\ \hline
% \multirow{4}{*}{}                                              &     & 956  & 331  & 68   & 140  \\ \cline{2-6} 
%                                                               &     & 0.34 & 0.47 & 0.70 & 0.85 \\ \cline{2-6} 
%                                                               &     & 0.31 & 0.35 & 0.38 & 0.93 \\ \cline{2-6} 
%                                                               &     & 4    & 4    & 4    & 4    \\ \hline
% \multirow{4}{*}{}                                              &     & 579  & 215  & 59   & 37   \\ \cline{2-6} 
%                                                               &     & 0.38 & 0.46 & 0.58 & 0.91 \\ \cline{2-6} 
%                                                               &     & 0.36 & 0.34 & 0.25 & 0.62 \\ \cline{2-6} 
%                                                               &     & 2    & 2    & 2    & 2    \\ \hline
% \multirow{4}{*}{}                                              &     & 546  & 220  & 56   & 66   \\ \cline{2-6} 
%                                                               &     & 0.24 & 0.30 & 0.43 & 0.56 \\ \cline{2-6} 
%                                                               &     & 0.25 & 0.25 & 0.28 & 0.83 \\ \cline{2-6} 
%                                                               &     & 2    & 2    & 2    & 3    \\ \hline
% \multirow{4}{*}{}                                              &     & 939  & 343  & 66   & 32   \\ \cline{2-6} 
%                                                               &     & 0.49 & 0.55 & 0.75 & 0.96 \\ \cline{2-6} 
%                                                               &     & 0.52 & 0.50 & 0.50 & 0.95 \\ \cline{2-6} 
%                                                               &     & 2    & 2    & 2    & 2    \\ \hline
% \multirow{4}{*}{}                                              &     & 141  & 95   & 47   & 10   \\ \cline{2-6} 
%                                                               &     & 0.39 & 0.39 & 0.54 & 0.99 \\ \cline{2-6} 
%                                                               &     & 0.34 & 0.33 & 0.28 & 1.00 \\ \cline{2-6} 
%                                                               &     & 1    & 1    & 1    & 1    \\ \hline
% \multirow{4}{*}{}                                              &     & 802  & 301  & 60   & 45   \\ \cline{2-6} 
%                                                               &     & 0.07 & 0.16 & 0.13 & 1.00 \\ \cline{2-6} 
%                                                               &     & 0.06 & 0.11 & 0.11 & 1.00 \\ \cline{2-6} 
%                                                               &     & 1    & 1    & 1    & 1    \\ \hline
% \end{tabular}%
% \end{table*}








% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\centering
%\scriptsize
\setlength{\tabcolsep}{2pt}
%\fontsize{9}{11}\selectfont
\begin{tabular}{|l|l|c|c|c|c|}
\hline
\multicolumn{6}{|c|}{Planar Segmentation  }                                                                                                                                                               \\ \hline
                                                                &     & MGS                              & ITKSF                               & DHF                               & DGS                                \\ \hline
                                                                & abc & {\color[HTML]{000000} 620}    & {\color[HTML]{000000} 218}    & {\color[HTML]{000000} 55}     & {\color[HTML]{000000} 34}      \\ \cline{2-6} 
                                                                & def & {\color[HTML]{000000} 9.8}  & {\color[HTML]{000000} 16.7} & {\color[HTML]{000000} 15.9} & {\color[HTML]{000000} 86.6}  \\ \cline{2-6} 
                                                                & ghi & {\color[HTML]{000000} 6.0}  & {\color[HTML]{000000} 7.6}  & {\color[HTML]{000000} 8.4}  & {\color[HTML]{000000} 84.6}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
} & jkl & {\color[HTML]{000000} 1}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}       \\ \hline
                                                                &     & {\color[HTML]{000000} 463}    & {\color[HTML]{000000} 201}    & {\color[HTML]{000000} 61}     & {\color[HTML]{000000} 57}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 18.3} & {\color[HTML]{000000} 26.8} & {\color[HTML]{000000} 44.8} & {\color[HTML]{000000} 96.1}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 16.7} & {\color[HTML]{000000} 21.3} & {\color[HTML]{000000} 31.2} & {\color[HTML]{000000} 100.0} \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}       \\ \hline
                                                                &     & {\color[HTML]{000000} 611}    & {\color[HTML]{000000} 231}    & {\color[HTML]{000000} 56}     & {\color[HTML]{000000} 64}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 16.0} & {\color[HTML]{000000} 23.9} & {\color[HTML]{000000} 27.5} & {\color[HTML]{000000} 81.8}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 11.7} & {\color[HTML]{000000} 12.5} & {\color[HTML]{000000} 15.0} & {\color[HTML]{000000} 82.2}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 3}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 3}       \\ \hline
                                                                &     & {\color[HTML]{000000} 956}    & {\color[HTML]{000000} 331}    & {\color[HTML]{000000} 68}     & {\color[HTML]{000000} 140}     \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 34.3} & {\color[HTML]{000000} 47.4} & {\color[HTML]{000000} 70.2} & {\color[HTML]{000000} 84.8}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 31.4} & {\color[HTML]{000000} 34.6} & {\color[HTML]{000000} 37.8} & {\color[HTML]{000000} 92.8}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 4}      & {\color[HTML]{000000} 4}      & {\color[HTML]{000000} 4}      & {\color[HTML]{000000} 4}       \\ \hline
                                                                &     & {\color[HTML]{000000} 579}    & {\color[HTML]{000000} 215}    & {\color[HTML]{000000} 59}     & {\color[HTML]{000000} 37}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 38.3} & {\color[HTML]{000000} 46.1} & {\color[HTML]{000000} 58.4} & {\color[HTML]{000000} 90.8}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 36.5} & {\color[HTML]{000000} 34.3} & {\color[HTML]{000000} 24.5} & {\color[HTML]{000000} 61.6}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}       \\ \hline
                                                                &     & {\color[HTML]{000000} 546}    & {\color[HTML]{000000} 220}    & {\color[HTML]{000000} 56}     & {\color[HTML]{000000} 66}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 23.6} & {\color[HTML]{000000} 30.3} & {\color[HTML]{000000} 42.7} & {\color[HTML]{000000} 56.3}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 24.6} & {\color[HTML]{000000} 25.0} & {\color[HTML]{000000} 28.3} & {\color[HTML]{000000} 83.1}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 3}       \\ \hline
                                                                &     & {\color[HTML]{000000} 939}    & {\color[HTML]{000000} 343}    & {\color[HTML]{000000} 66}     & {\color[HTML]{000000} 32}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 48.8} & {\color[HTML]{000000} 55.2} & {\color[HTML]{000000} 74.8} & {\color[HTML]{000000} 95.7}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 51.9} & {\color[HTML]{000000} 49.6} & {\color[HTML]{000000} 50.0} & {\color[HTML]{000000} 95.2}  \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}      & {\color[HTML]{000000} 2}       \\ \hline
                                                                &     & {\color[HTML]{000000} 141}    & {\color[HTML]{000000} 95}     & {\color[HTML]{000000} 47}     & {\color[HTML]{000000} 10}      \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 38.5} & {\color[HTML]{000000} 39.1} & {\color[HTML]{000000} 53.6} & {\color[HTML]{000000} 99.3}  \\ \cline{2-6} 
                                                                &     & {\color[HTML]{000000} 33.9} & {\color[HTML]{000000} 33.3} & {\color[HTML]{000000} 27.5} & {\color[HTML]{000000} 100.0} \\ \cline{2-6} 
\multirow{-4}{*}{
\begin{tabular}{c{5cm}}
     \includegraphics[width=5.3cm,height=1.5cm]{hyp_images/abc.pdf} \vspace{-0.24cm} \\
     Barrsmith, N=600
     \vspace{-0.24cm}\\
     O=\%65.4, \tau=3, $S=[50,20,23,34,45]$\\
\end{tabular}
}                                              &     & {\color[HTML]{000000} 1}      & {\color[HTML]{000000} 1}      & {\color[HTML]{000000} 1}      & {\color[HTML]{000000} 1}       \\ \hline
\end{tabular}%
\end{table*}

==> old_hyp_gen_combined.tex <==
\begin{table*}[h!]
\label{tab:kdgs_quan}
\centering
\scriptsize
\caption{\textbf{Guided Hypothesis Generation Comparison:} \#H number of hypotheses generated, \#HM(\%) percentage of all inlier MSS, \#HI(\%) percentage of hypotheses having at-least 80\% overlap of their estimated inliers with the true inliers, $n$: number of point correspondences, O(\%) outlier percentage. The $S$ vector shows the number of points belong to per true structure. \textit{tim}(s) time taken in seconds.}
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|ccccc||c|ccccc|}
\hline
\multicolumn{6}{|c||}{\textbf{Planar Segmentation}}                                                                                                                                                                                                          & \multicolumn{6}{c|}{\textbf{Motion Segmentation}}                                                                                                                                                                                                       \\ \hline
                                                          Data      &     &  MGS                                    &       ITKSF                            &           DHF                          &   DGS                                      &                                  Data                               &     &                           MGS     &                           ITKSF     &          DHF                               & DGS                                        \\ \hline
                                                                & \#H & { 620}          & { 218}        & { 55}           & { 34}               &                                                                 & \#H & { 380}     & { 213}     & { 68}               & { 154}              \\
                                                                & \#HM & { 9.8}          & { {\ul 16.7}} & { 15.9}         & { \textbf{86.6}}    &  & \#HM & { 32.15} & { 57.98} & { {\ul 85.23}}    & {\textbf{86.39}} \\   & \#HI & { 6.0}          & { 7.6}        & { {\ul 8.4}}    & { \textbf{84.6}}    &                 & \#HI & { 55.69} & { 59.41} & { {\ul 73.79}}    & { \textbf{97.30}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/barrsmith.pdf} \vspace{-.2cm} \\
     barrsmith, N~=~235, O~=~69.8\%
     \vspace{-0.15cm}\\
     S~=~[~50,21~]\\
\end{tabular}} & tim & { 1}            & { 2}          & { 2}            & { 2}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/biscuitbookbox.pdf} \vspace{-.2cm} \\
     biscuitbookbox, N~=~258, O~=~37.2\%
     \vspace{-0.15cm}\\
     S~=~[~67,41,54~]\\
\end{tabular}} & tim & { 3}       & { 3}       & { 3}                & { 3}                \\
      & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline

                                              & \#H & { 463}          & { 201}        & { 61}           & { 57}               &                                                                 & \#H & { 328}     & { 169}     & { 71}               & { 157}              \\ 
                                                                & \#HM & { 18.3}       & { 26.8}     & { {\ul 44.8}} & { \textbf{96.1}}  &                                                                 & \#HM & { 21.67} & { 32.26} & { {\ul 68.34}}    & { \textbf{69.41}} \\ 
                                                                & \#HI & { 16.7}       & { 21.3}     & { {\ul 31.2}} & { \textbf{100.0}} &                                                                 & \#HI & { 44.92} & { 41.50} & { {\ul 75.53}}    & { \textbf{95.83}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/elderhalla.pdf} \vspace{-.2cm} \\
     elderhalla,~~~N~=~214,~O~=~60.8\%
     \vspace{-0.15cm}\\
     S~=~[~38,~46~]\\
\end{tabular}}                                              & tim & { 2}            & { 2}          & { 2}            & { 2}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/boardgame.pdf} \vspace{-.2cm} \\
     boardgame, N~=~266,~O~=~42.5\%
     \vspace{-0.15cm}\\
     S~=~[~63,~63,~27~]\\
\end{tabular}}                                              & tim & { 3}       & { 3}       & { 3}                & { 3}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 611}          & { 231}        & { 56}           & { 64}               &                                                                 & \#H & { 264}     & { 182}     & { 68}               & { 130}              \\ 
                                                                & \#HM & { 16.0}       & { 23.9}     & { {\ul 27.5}} & { \textbf{81.8}}  &                                                                 & \#HM & { 21.79} & { 50.14} & { \textbf{72.31}} & { {\ul 67.53}}    \\ 
                                                                & \#HI & { 11.7}       & { 12.5}     & { {\ul 15.0}} & { \textbf{82.2}}  &            & \#HI & { 46.00} & { 73.66} & { {\ul 94.45}}    & { \textbf{96.87}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/elderhallb.pdf} \vspace{-.2cm} \\
     elderhallb, N~=~245,~O~=~49.8\%
     \vspace{-0.15cm}\\
     S~=~[~	38,~25,~60~]\\
   %  elderhallb.mat'	245	49.8%	122	38	25	60
\end{tabular}}                                              & tim & { 2}            & { 3}          & { 2}            & { 3}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/breadcartoychips.pdf} \vspace{-.2cm} \\
     breadcartoychips, N~=~231, O~=~35.5\%
     \vspace{-0.15cm}\\
     S~=~[~33,~23,~39,~54~]\\
    % breadcartoychips.mat'	231	35.5%	82	33	23	39	54
\end{tabular}}                                              & tim & { 4}       & { 4}       & { 4}                & { 4}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 956}          & { 331}        & { 68}           & { 140}              &                                                                 & \#H & { 258}     & { 181}     & { 70}               & { 137}              \\  
                                                                & \#HM & { 34.3}       & { 47.4}     & { {\ul 70.2}} & { \textbf{84.8}}  &                                                                 & \#HM & { 27.26} & { 55.98} & { \textbf{86.98}} & { {\ul 76.68}}    \\ 
                                                                & \#HI & { 31.4}       & { 34.6}     & { {\ul 37.8}} & { \textbf{92.8}}  &                                                                 & \#HI & { 52.40} & { 73.70} & { {\ul 89.16}}    & { \textbf{96.24}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/johnsona.pdf} \vspace{-.2cm} \\
     johnsona, N~=~353,~O~=~21.2\%
     \vspace{-0.15cm}\\
     S~=~[~76,~91,~61,~50~]\\
   %  johnsona.mat'	353	21.2%	75	76	91	61	50
\end{tabular}}                                              & tim & { 4}            & { 4}          & { 4}            & { 4}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/breadcubechips.pdf} \vspace{-.2cm} \\
     breadcubechips, N~=~230, O~=~35.2\%
     \vspace{-0.15cm}\\
     S~=~[~34,~57,~58~]\\
   %  breadcubechips.mat'	230	35.2%	81	34	57	58
\end{tabular}}                                              & tim & { 3}       & { 3}       & { 3}                & { 3}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 579}          & { 215}        & { 59}           & { 37}               &                                                                 & \#H & { 415}     & { 237}     & { 76}               & { 81}               \\ 
                                                                & \#HM & { 38.3}       & { 46.1}     & { {\ul 58.4}} & { \textbf{90.8}}  &                                                                 & \#HM & { 28.30} & { 51.56} & { \textbf{85.66}} & { {\ul 80.29}}    \\                    & \#HI & { {\ul 36.5}} & { 34.3}     & { 24.5}       & { \textbf{61.6}}  &                                                                 & \#HI & { 58.80} & { 67.77} & { {\ul 90.56}}    & { \textbf{97.29}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/ladysymon.pdf} \vspace{-.2cm} \\
     ladysymon, N~=~227, O~=~33.5\%
     \vspace{-0.15cm}\\
     S~=~[~102,~49~]\\
    % ladysymon.mat'	227	33.5%	76	102	49
\end{tabular}}                                              & tim & { 2}            & { 2}          & { 2}            & { 2}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/breadtoy.pdf} \vspace{-.2cm} \\
     breadtoy, N~=~278, O~=~37.4\%
     \vspace{-0.15cm}\\
     S~=~[~119,~55~]\\
    % breadtoy.mat'	278	37.4%	104	119	55
\end{tabular}}                                              & tim & { 2}       & { 2}       & { 2}                & { 2}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 546}          & { 220}        & { 56}           & { 66}               &                                                                 & \#H & { 197}     & { 135}     & { 57}               & { 88}               \\ 
                                                                & \#HM & { 23.6}       & { 30.3}     & { {\ul 42.7}} & { \textbf{56.3}}  &                                                                 & \#HM & { 21.55} & { 50.67} & { {\ul 71.31}}    & { \textbf{75.12}} \\ 
                                                                & \#HI & { 24.6}       & { 25.0}     & { {\ul 28.3}} & { \textbf{83.1}}  &                                                                 & \#HI & { 40.44} & { 66.58} & { {\ul 82.22}}    & { \textbf{96.82}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/napierb.pdf} \vspace{-.2cm} \\
     napierb, N~=~237, O~=~37.1\%
     \vspace{-0.15cm}\\
     S~=~[~46,~33,~70~]\\
    % napierb.mat'	237	37.1%	88	46	33	70
\end{tabular}}                                              & tim & { 2}            & { 2}          & { 2}            & { 3}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/breadtoycar.pdf} \vspace{-.2cm} \\
     breadtoycar, N~=~164, O~=~34.1\%
     \vspace{-0.15cm}\\
     S~=~[~37,~39,~32~]\\
  %   breadtoycar.mat'	164	34.1%	56	37	39	32
\end{tabular}}                                              & tim & { 3}       & { 3}       & { 3}                & { 3}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 939}          & { 343}        & { 66}           & { 32}               &                                                                 & \#H & { 176}     & { 138}     & { 57}               & { 84}               \\ 
                                                                & \#HM & { 48.8}       & { 55.2}     & { {\ul 74.8}} & { \textbf{95.7}}  &                                                                 & \#HM & { 23.64} & { 50.37} & { {\ul 69.42}}    & { \textbf{70.21}} \\ 
                                                                & \#HI & { {\ul 51.9}} & { 49.6}     & { 50.0}       & { \textbf{95.2}}  &                                                                 & \#HI & { 50.37} & { 69.12} & { {\ul 84.95}}    & { \textbf{92.86}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/oldclassicswing.pdf} \vspace{-.2cm} \\
     oldclassicswing, N~=~363, O~=~32.2\%
     \vspace{-0.15cm}\\
     S~=~[~181,~65~]\\
    % oldclassicswing.mat'	363	32.2%	117	181	65
\end{tabular}}                                              & tim & { 2}            & { 2}          & { 2}            & { 2}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/carchipscube.pdf} \vspace{-.2cm} \\
     carchipscube, N~=~164, O~=~36.6\%
     \vspace{-0.15cm}\\
     S~=~[~18,~33,~53~]\\
  %   carchipscube.mat'	164	36.6%	60	18	33	53
\end{tabular}}                                              & tim & { 3}       & { 3}       & { 3}                & { 3}                \\ & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
                                                                & \#H & { 141}          & { 95}         & { 47}           & { 10}               &                                                                 & \#H & { 371}     & { 191}     & { 73}               & { 170}              \\  
                                                                & \#HM & { 38.5}       & { 39.1}     & { {\ul 53.6}} & { \textbf{99.3}}  &                                                                 & \#HM & { 21.53} & { 36.11} & { \textbf{86.73}} & { {\ul 74.94}}    \\ 
                                                                & \#HI & { {\ul 33.9}} & { 33.3}     & { 27.5}       & { \textbf{100.0}} &                                                                 & \#HI & { 42.67} & { 48.17} & { {\ul 81.37}}    & { \textbf{98.10}} \\ 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/physics.pdf} \vspace{-.2cm} \\
     physics, N~=~103, O~=~46.6\%
     \vspace{-0.15cm}\\
     S~=~[~55~]\\
  %   physics.mat'	103	46.6%	48	55
\end{tabular}}                                              & tim & { 1}            & { 1}          & { 1}            & { 1}                & \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
     \includegraphics[width=4cm,height=1.5cm]{hyp_images/cubechips.pdf} \vspace{-.2cm} \\
     cubechips, N~=~277, O~=~51.6\%
     \vspace{-0.15cm}\\
     S~=~[~81,~53~]\\
   %  cubechips.mat'	277	51.6%	143	81	53
\end{tabular}}                                              & tim & { 2}       & { 2}       & { 2}                & { 2}                \\       & &          &         &           &              &                                                                 & &      &      &               &               \\
       \hline
\end{tabular}
}
\end{table*}

==> old_point_preferences.tex <==
% \begin{table*}[h]
% \centering
\begin{figure*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllllll}
%\hline
\multicolumn{3}{l}{\multirow{5}{*}{\hspace{-0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=2.5cm,height=2.5cm]{./images/res_corr.pdf}\\\hspace{-0.25cm}(a)\end{tabular}}} & \multicolumn{3}{l}{\multirow{5}{*}{\hspace{0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=2.5cm,height=2.5cm]{./images/den_corr.pdf}\\(b)\end{tabular}}} & \multicolumn{3}{l}{\multirow{5}{*}{\hspace{0.3cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=3.5cm]{./images/zero_corr_1_rd.pdf}\\\hspace{0.3cm}(c)\end{tabular}}} & \multicolumn{3}{l}{\multirow{5}{*}{\hspace{1.1cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=3.5cm]{./images/zero_corr_2_rd.pdf}\\\hspace{1.1cm}(d)\end{tabular}}} & \multicolumn{3}{l}{\multirow{5}{*}{\hspace{-0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=3.5cm]{./images/zero_corr_3_rd.pdf}\\(e)\end{tabular}}} & \multirow{5}{*}{} & \multicolumn{4}{l}{\multirow{12}{*}{\hspace{-0.4cm}\vspace{5cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=3.7cm]{hyp_images/time_vs_pts.eps}\\(n)\end{tabular}}} \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{\multirow{3}{*}{\hspace{-0.1cm} \begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/res_st0.pdf}\\(f)\end{tabular}}}                                              & \multicolumn{4}{l}{\multirow{3}{*}{\hspace{-0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/res_st1.pdf}\\(g)\end{tabular}}}                & \multicolumn{4}{l}{\multirow{3}{*}{\hspace{-0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/res_st2.pdf}\\(h)\end{tabular}}}               & \multicolumn{4}{l}{\multirow{3}{*}{\hspace{-0.0cm}\begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/res_st3.pdf}\\(i)\end{tabular}}}                     & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{}                                                                             & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                       & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{}                                                                             & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                       & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
\multicolumn{3}{l}{}                                                               & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   & \multicolumn{3}{l}{}                   &                   & \multicolumn{4}{l}{}                    \\
%\cline{1-16}
\multicolumn{4}{l}{\multirow{4}{*}{\hspace{-0.1cm} \begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/den_st0.pdf}\\(j)\end{tabular}}}                                                               & \multicolumn{4}{l}{\multirow{4}{*}{\hspace{-0.0cm} \begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/den_st1.pdf}\\(k)\end{tabular}}}                 & \multicolumn{4}{l}{\multirow{4}{*}{\hspace{-0.0cm} \begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/den_st2.pdf}\\(l)\end{tabular}}}                & \multicolumn{4}{l}{\multirow{4}{*}{\hspace{-0.0cm} \begin{tabular}[c]{@{}c@{}}\includegraphics[width=4.7cm]{./images/den_st3.pdf}\\(m)\end{tabular}}}                     & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{}                                                                             & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                       & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{}                                                                             & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                       & \multicolumn{4}{l}{}                    \\
\multicolumn{4}{l}{}                                                                             & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                 & \multicolumn{4}{l}{}                                       & \multicolumn{4}{l}{}                    \\ %\hline
\end{tabular}
}
%\vspace{-0.8cm}
	\caption{\small \textbf{Residual vs. Density based point correlation}: $breadcubechips$ sequence of AdelaideRMF  \cite{wong2011dynamic} dataset (a) Residual based and (b) Density based point correlation matrix with rows and columns ordered by structure membership. (c), (d) and (e) are percentage of \emph{uncorrelated} outliers varying with iterations of (Algo. \ref{dgs}) for each of the three structures $bread$, $cube$ and $chips$ respectively. Rows 2  and 3 show structure-wise averaged correlation (see Sec. \ref{sec:pt_pref}) for details.}%
\end{figure*}
%\end{table*}

==> qual_hom.tex <==
\begin{figure*}[h]
\centering
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccccc}
& elderhalla & johnsona & library & ladysymon & sene \\
 \rotatebox{90}{\hspace{.2cm}  \textbf{GroundTruth}} &    \includegraphics[width=2.6cm]{qualitative_imgs/hom_1_gt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_2_gt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_3_gt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_4_gt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_5_gt.pdf} \\
  \rotatebox{90}{\hspace{.2cm}  \textbf{DGSAC-G}}   & \includegraphics[width=2.6cm]{qualitative_imgs/hom_1_grdy.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_2_grdy.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_3_grdy.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_4_grdy.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_5_grdy.pdf} \\
   \rotatebox{90}{\hspace{.2cm}  \textbf{DGSAC-O}}      &\includegraphics[width=2.6cm]{qualitative_imgs/hom_1_opt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_2_opt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_3_opt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_4_opt.pdf}&
     \includegraphics[width=2.6cm]{qualitative_imgs/hom_5_opt.pdf} \\
\end{tabular}
\caption{\textbf{Some Qualitative Results of Planar Segmentation.} Qualitative results are shown for some examples from AdelaideRMF \cite{wong2011dynamic} dataset}
\end{figure*}
